Loan maturity aggregation in interbank lending networks obscures mesoscale structure and economic functions

Since the 2007-2009 financial crisis, substantial academic effort has been dedicated to improving our understanding of interbank lending networks (ILNs). Because of data limitations or by choice, the literature largely lacks multiple loan maturities. We employ a complete interbank loan contract dataset to investigate whether maturity details are informative of the network structure. Applying the layered stochastic block model of Peixoto (2015) and other tools from network science on a time series of bilateral loans with multiple maturity layers in the Russian ILN, we find that collapsing all such layers consistently obscures mesoscale structure. The optimal maturity granularity lies between completely collapsing and completely separating the maturity layers and depends on the development phase of the interbank market, with a more developed market requiring more layers for optimal description. Closer inspection of the inferred maturity bins associated with the optimal maturity granularity reveals specific economic functions, from liquidity intermediation to financing. Collapsing a network with multiple underlying maturity layers or extracting one such layer, common in economic research, is therefore not only an incomplete representation of the ILN's mesoscale structure, but also conceals existing economic functions. This holds important insights and opportunities for theoretical and empirical studies on interbank market functioning, contagion, stability, and on the desirable level of regulatory data disclosure.

==> appendices/evidence.tex <==
\section{Evidence-based OG inference}

\begin{figure}[h] 
\centering
\includegraphics{suppl/evidence.pdf}
\caption{Results of the layered SBM with evidence collection. (a) Posterior odds ratios of the OLP compared to two other main cases corresponding resp. to the highest and lowest possible maturity granularity: all layers separate and complete maturity collapse. The latter, though most often used, is always suboptimal to the OLP. (b) The OLP. Maturities with equal color are part of the same (merged) layer in the OLP, also indicated by the number (the Optimal Layer index or OLi).\label{contiguous-evidence}}
\end{figure}

% OLD EVIDENCE NOTES

% Alternatively, ...
% Evidence approach: explain and refer to Appendix C. If evidence approach does not work, perhaps explain why in a subsubsection here and try to figure out why we should be OK with inferring all simultaneously

% OLD NOTES:
% - Optimal granularity based on evidence. Evidence can be only based on RUN9. We take just the minimum DL because (a) is easier to understand because of the similarity to an objective function based approach; (b) The evidence approach rests on the Bethe approximation which requires locally non-tree behavior, a condition not readily satisfied by the network; (c) Because we are searching a non-continuous state space, there are no problems with typicality etc. (We are not optimizing for probability density but for probability mass. But is this actually relevant here?) (d) There are indications of a unimodal pdf over the bank groups. So looking for its maximum is quite sensible.

==> tbl/role-exp-matrix.tex <==
\begin{tabular}{c|c|c|c|l}
                                   &          &          &    &  \\ \hline
LO                                 & 0        & 0        & 0  &  \\ \hline
IM                                 & 0 & $\geq 0$ & $\geq 0$   &  \\ \hline
BO                                 & 0 & $\geq 0$ & $\geq 0$   &  \\ \hline
$\nwarrow$ & BO       & IM       & LO & 
\end{tabular}
\ $\longrightarrow$ \ 
\begin{tabular}{c|c|c|c}
                                   &      &      &  \\ \hline
IM                                 & $>0$ & $>0$ &  \\ \hline
BO                                 & $\approx 0$    & $>0$ &  \\ \hline
$\nwarrow$ & LO   & IM   & 
\end{tabular}

==> tbl/stylized-facts.tex <==
\begin{tabular}{@{}llll@{}}
\toprule
ILN measure   & Value & Layer homogeneity  & Selected studies \\ \midrule
density                      & \textbf{sparse}  & No        & \cite{Finger2013,Huser2015,aldasoro2016,Blasques2018,silva2015,bargigli2015}        \\
degree distribution (in and out degrees)          & \textbf{heavy-tailed} & Yes   &  \cite{Finger2013,Huser2015,aldasoro2016,Vandermarliere2015,bargigli2015,Craig2014}       \\
topology                     & scale-free / core-periphery & No &\cite{demasi2006,soramaki2006,bargigli2015}/\cite{Huser2015,Craig2014,aldasoro2016,Blasques2018,silva2015} \\
clustering coefficients      & low / \textbf{high} & No   &  \cite{Finger2013}/\cite{Huser2015,aldasoro2016,soramaki2006,bargigli2015} \\
average shortest path length & \textbf{small} / "small world" & No   &  \cite{aldasoro2016,silva2015}/ \cite{Finger2013,Huser2015,soramaki2006}       \\
bank size mixing             & \textbf{disassortative} & No & \cite{Finger2013,Huser2015,aldasoro2016,demasi2006,silva2015,borboa2015}       \\
distribution of transaction volumes           & \textbf{heavy-tailed}   & Yes & \cite{Finger2013,Vandermarliere2015}       \\ \bottomrule
\end{tabular}
